Optimal Repair For Omega-regular Properties

This paper presents an optimization based framework to automate system repair against omega-regular properties. In the proposed formalization of optimal repair, the systems are represented as Kripke structures, the properties as $\omega$-regular languages, and the repair space as repair machines -- weighted omega-regular transducers equipped with B\"uchi conditions -- that rewrite strings and associate a cost sequence to these rewritings. To translate the resulting cost-sequences to easily interpretable payoffs, we consider several aggregator functions to map cost sequences to numbers -- including limit superior, supremum, discounted-sum, and average-sum -- to define quantitative cost semantics. The problem of optimal repair, then, is to determine whether traces from a given system can be rewritten to satisfy an $\omega$-regular property when the allowed cost is bounded by a given threshold. We also consider the dual challenge of impair verification that assumes that the rewritings are resolved adversarially under some given cost restriction, and asks to decide if all traces of the system satisfy the specification irrespective of the rewritings. With a negative result to the impair verification problem, we study the problem of designing a minimal mask of the Kripke structure such that the resulting traces satisfy the specifications despite the threshold-bounded impairment. We dub this problem as the mask synthesis problem. This paper presents automata-theoretic solutions to repair synthesis, impair verification, and mask synthesis problem for limit superior, supremum, discounted-sum, and average-sum cost semantics.

==> mask-synthesis.tex <==
\subsection{Mask Synthesis}
Given the Kripke structure $K$ representing the system, a repair machine $T$, and a threshold $v$, the Mask synthesis problem is to find a subset $N' \subseteq K$ of traces for which the corresponding repair policy problem can be solved.
\\~\\
We show the following:
\begin{itemize}
    \item [(a)] The subset $N'$ is $\omega$-regular for the $\mathsf{Sup}, \mathsf{LimSup}$ aggregator functions.
    \item [(b)] The subset $N'$ is $\omega$-regular for the $\mathsf{DSum}$-aggregator function if $K$ is cut-point regular.
    \item [(c)] We leave the problem open for the $\mathsf{Mean}$-aggregator function.
\end{itemize}

==> mask-verification.tex <==
\subsection{Mask Synthesis}
It is well known that every Kripke structure admits an $\omega$-regular $N$ such that a word $u \in N$ if and only if $u \in \Tt_K$. 
Let the $\omega$-regular language of $K$ be $N$.
To solve the mask synthesis problem, we restrict the domain of the repair machine $T$ to $N$ by constructing a repair machine $T'$ using product construction and give our results on the repair machine $T'$.


%In the proofs for $\omega$-regular kernels, we make use of lemma 14 from \cite{concur20} and extend this to $\omega$-regular words. 

%% 	That is, given a threshold $v$, $\omega$-regular language $L$ defined by an NBA $A$, and a \buchi transducer $T$, we have $\overline{Rob_T(v,L)} = \{ w_1, \mid \exists w_2, C_T(w_1,w_2) < v , w_2 \notin L \}$ to be $\omega$-regular when the cost function $C$ is the $\mathsf{Sup}$ or $\mathsf{LimSup}$ aggregator function.  
%% Similar to \cite{concur20}, we simulate $T$ over $L$ and reject if the word written by $T$ is in $L$, and achieve this by taking the product of $T$ with the NBA of $\overline{A}$ and run the NBA $\overline{A}$ corresponding to language $\overline{L}$ on the output of $T$, so $\overline{Rob_T(v,L)} = \{ w_1, \mid \exists w_2, C_{T \otimes \overline{A} }(w_1,w_2) < v \}$. 
%% Lastly, we note that the language $L(A^{\geq v}) = \{ w \mid U(w) \geq v \}$ for a  $\mathsf{Sup}$ or a $\mathsf{LimSup}$ automata $U$ is $\omega$-regular to complete the extension. 

%\subsection{Sum aggregator function}
%As in the verification case, if the transducer $T$ happens to have no accepting cycles with a total cost of $0$, the robust kernel for the Sum aggregator function is empty for all values of $v$ that are not $\infty$. 
%%and the robust kernel is $\Sigma^{\omega}$ otherwise. 
%If there is an accepting cycle with a total cost of $0$, then we have $u \in Rob_T(v,L)$ iff there exists a path of cost at most $v$ that starts from the initial state and reaches the accepting cycle of cost $0$.
%This check can easily be done by storing the cost upto $v$ in the finite control state.


%\subsection{DSum$_\lambda$ aggregator function}
%\label{subsec:dsum-kernel}
%We give the partial answer for this function.
\subsubsection{Mask Synthesis for $DSum$-RMs.} 
We show that the maximal subset $N'$ for isolated cut-point languages is $\omega$-regular.
%The concept of cut-point language comes from the theory of probabilistic automata. 
Given a threshold $\tau \in \Qq$, the maximal subset $N'$, is the set of all words $u \in \dom(T')$, such that for every word $w' \in \sem{T}^{\mathsf{DSum}}_{\tau}(u)$ we also have $w \notin L$.
%It is known that for $\epsilon$-isolated threshold, the cut point languages are regular~\cite{ExpressivenessQL}.
A threshold $\tau$ is $\epsilon$-isolated for repair machine $T'$, if for $\epsilon > 0$ and all accepting runs $r$ of $T'$, $\sem{T'}^{\mathsf{DSum}}_{*}(r,w) \in [0, v-\epsilon] \cup [v+\epsilon, \infty)$. 
It is isolated if it is isolated for some $\epsilon$.
To prove that $N'$ is $\omega$-regular for such thresholds, we first note that isolated-cut point languages are $\omega$-regular in the context of weighted automata~\cite{ExpressivenessQL}.
We follow a similar strategy to~\cite{concur20}, and slowly unroll our synchronous product.
We note that since the repair machine is over $\omega$ strings, there must exist some $n$ such that $\mathsf{DSum}(w_0 w_1 \ldots) \leq \mathsf{DSum}(w_0 \ldots w_n) + B_n$, where $B_n = V \frac{\lambda^{n}}{1-\lambda}$, where $V$ is the largest cost that is not $\infty$. Therefore if $\mathsf{DSum}(w_0, w_1, \ldots) \leq v - \epsilon + B_n$ we can conclude that $\mathsf{DSum}(w_0, \ldots, w_n) \leq v - \epsilon$.    

%We therefore extend lemmas 18 and 19 from \cite{concur20}:
\begin{lemma}\label{lem:dsum1}
	Let $T'$ be a $\dsum$-RM  and $\tau \in \Qq$. 
	If $\tau$ is $\epsilon$-isolated for some $\epsilon$, then there is $n^* \in \Nn$ such that any partial run $r$ of length at least $n^{*}$ satisfies one of the following properties:
	\begin{enumerate}
		\item $\dsum(r) {\leq} \tau {-} \epsilon$ and $\dsum(rr') {\leq} \tau {-} \epsilon$ for every 		infinite continuation $r'$ of $r$.
		\item $\dsum(r) {\geq} \tau {+} \frac{\epsilon}{2}$ and $\dsum(rr') {\geq} \tau{+} \epsilon$ for every infinite continuation $r'$ of $r$.
	\end{enumerate}
	Here, for finite $r$, $\dsum(r)$ is defined in the usual fashion except that the summation will be upto the length of $r$.
\end{lemma}

\begin{theorem}
	\label{thm:dsum2}
	Let $T'$ be a $\dsum$-RM, $v \in \Qq$, and $L$ an $\omega$-regular language given by
	an NBA. For all $n$, we can construct an NBA $A_n$ such that 
        $L(A_n) \subseteq L(A_{n+1})$ and
	$L(A_n) \subseteq \overline{N'} \cap \dom(T')$. 
	%% \begin{enumerate}
	%% 	\item $L(A_n) \subseteq L(A_{n+1})$
	%% 	\item $L(A_n) \subseteq \overline{Rob_T(v,L)} \cap \dom(T)$
	%% \end{enumerate}
	Moreover, if $\tau$ is $\epsilon$-isolated, there exists $n^*$ such that $L(A_{n^*}) = \overline{N'} \cap \dom(T')$. 
\end{theorem}
%The proof of Lemma~\ref{lem:dsum1} is by simple calculations (Proof in Appendix~\ref{app:lem-dsum1}).
%For Lemma~\ref{lem:dsum2}, we construct a sequence of NBAs $A_n$. % but the acceptance condition is based only on transducer $T$, not the bad runs. 
For the construction of $A_n$ in Theorem~\ref{thm:dsum2}, a notion of bad and dangerous runs are defined. 
Intuitively, The bad runs are all those runs which are accepting with cost $\leq \tau$, such that the output word is not in $L$.
The dangerous runs are the finite partial runs which can be extended to bad runs.
The idea for construction of $A_n$ is to identify all the finite partial runs $r$ of length $n$ which can later be extended to bad runs.
This way we can construct a sequence of \buchi automata that better under approximate the automata for the non-robust words in the domain.
Thanks to Lemma~\ref{lem:dsum1}, we can assure that there exists a fixed point at $n^*$ such that $A_{n^*}$ recognizes all the non-robust words from $T'$. Details are given in Appendix~\ref{app:verification}.


\subsubsection{Mask synthesis for $\supf$-RMs and $\limsupf$-RMs.}
For the $\mathsf{Sup}$-RMs, we note that we can construct an NBA recognizing all output words with a cost greater than $\tau$ via Lemma~\ref{lem:sup1} and show that the maximal subset $N'$ is $\omega$-regular. %(Proof in Appendix~\ref{app:lem-sup1})
\begin{lemma}\label{lem:sup1}
	Given a $\mathsf{Sup}$-automaton $U= (Q,q_i,\delta,\gamma)$ over $\Sigma^{\omega}$, %(defined in \cite{QuantitativeLanguagesKLT}), 
	and a rational number $\tau$, we can find an NBA  $A^{> \tau} = (Q^{> \tau}, q_i^{> \tau}, \delta^{> \tau}, F^{> \tau})$ such that 
	\[
	L(A^{> \tau}) = \{ w \mid U(w) > \tau \}.
	\]
\end{lemma}

\begin{theorem}\label{thm:sup-mask}
	Let $T'$ be a $\supf$-RM, $\tau \in \Qq$ and $L$ be a $\omega$-regular language. The language of $N'$ is $\omega$-regular and we can effectively construct an NBA for it.
\end{theorem}
We present the proof of this in the Appendix~\ref{app:sup-mask} using Lemma~\ref{lem:sup1}.
%\begin{proof}
%	We construct $A^{> v}$ as follows :
%	\begin{itemize}
%		\item [] $Q^{> v} = Q \times \{0,1\} $,
%		\item [] $q_i^{> v} = (q_i,0) $,
%		\item []$ ((q,i), \sigma , (p,j) ) \in \delta^{> v} $ if $(q, \sigma, p) \in \delta$ and one of the following is satisfied:
%		\begin{itemize}
%			\item $i = 0$, $j = 0$ and $ \gamma(q,p) \leq v$.
%			\item $i = 0$, $j = 1$ and $\gamma (q,p) > v$.
%			\item $i = 1$ and $j = 1$. 
%		\end{itemize}
%		\item $F^{> v} = Q^{> v} \times {1}$.
%	\end{itemize}
%	And observe that $A^{> v}$ accepts a word $w \in \Sigma^{\omega}$ iff $ U(w) > v$.
%\end{proof}
%%Alternatively we can use theorem 4 lemma 1 and convert any Sup automata to a LimSup automata and push the result through. 
%%We make use of this combined with the extension of lemma 14 from \cite{concur20} to arrive at an NBA for $\rob_T(v, L)$.
%Using the above lemma, we derive the following result. (Proof in Appendix~\ref{app:lem-sup})
%\begin{lemma}\label{lem:sup}
%	Let $T$ be a $\supf$-transducer, $v \in \Nn$ and $L$ is a regular language. The language of $\rob_T(v, L)$ is regular and we can effectively construct an NBA for it.
%\end{lemma}

%\subsection{LimSup aggregator function}
The results for $\supf$-RMs can be extended carefully to only account the costs occurring in accepting loops and be used for the $\limsupf$-RMs as well.
%For the LimSup aggregator function we make use of Theorem 4, Lemma 2 from \cite{QuantitativeLanguagesKLT} and the extension of lemma 14 from \cite{concur20} to arrive at an NBA for $\rob_T(v, L)$. 
%Thus, the non-emptiness of the robust kernel in the case of the DSum$_\lambda$, Sup, and LimSup aggregator function can be reduced to the problem of checking the non-emptiness of the correspondingly constructed \buchi automata.

%\subsection{Sup Aggregator function}
%For the $\mathsf{Sup}$ aggregator function we make use of the following lemma: 
%
%\begin{lemma}\label{lem:sup1}
%	Given a $\mathsf{Sup}$-automata $U= (Q,q_i,\delta,\gamma)$ over $\Sigma^{\omega}$, %(defined in \cite{QuantitativeLanguagesKLT}), 
%	and a rational number $v$, we can find an NBA  $A^{> v} = (Q^{> v}, q_i^{> v}, \delta^{> v}, F^{> v})$ such that $L(A^{> v}) = \{ w \mid U(w) > v \}$.
%\end{lemma}
%\begin{proof}
%	We construct $A^{> v}$ as follows :
%	\begin{itemize}
%		\item [] $Q^{> v} = Q \times \{0,1\} $,
%		\item [] $q_i^{> v} = (q_i,0) $,
%		\item []$ ((q,i), \sigma , (p,j) ) \in \delta^{> v} $ if $(q, \sigma, p) \in \delta$ and one of the following is satisfied:
%		\begin{itemize}
%			\item $i = 0$, $j = 0$ and $ \gamma(q,p) \leq v$.
%			\item $i = 0$, $j = 1$ and $\gamma (q,p) > v$.
%			\item $i = 1$ and $j = 1$. 
%		\end{itemize}
%		\item $F^{> v} = Q^{> v} \times {1}$.
%	\end{itemize}
%	And observe that $A^{> v}$ accepts a word $w \in \Sigma^{\omega}$ iff $ U(w) > v$.
%\end{proof}
%%Alternatively we can use theorem 4 lemma 1 and convert any Sup automata to a LimSup automata and push the result through. 
%%We make use of this combined with the extension of lemma 14 from \cite{concur20} to arrive at an NBA for $\rob_T(v, L)$.
%Using the above lemma, we derive the following result. (Proof in Appendix~\ref{app:lem-sup})
%\begin{lemma}\label{lem:sup}
%	Let $T$ be a $\supf$-transducer, $v \in \Nn$ and $L$ is a regular language. The language of $\rob_T(v, L)$ is regular and we can effectively construct an NBA for it.
%\end{lemma}
%
%\subsection{LimSup aggregator function}
%The results for $\sup$ aggregator functions can be extended carefully to only account the costs occurring in accepting loops.
%%For the LimSup aggregator function we make use of Theorem 4, Lemma 2 from \cite{QuantitativeLanguagesKLT} and the extension of lemma 14 from \cite{concur20} to arrive at an NBA for $\rob_T(v, L)$. 
%
%Thus, to solve the non-emptiness problem in the case of the DSum$_\lambda$, Sup, and LimSup aggregator function, we need to check the non-emptiness of the correspondingly constructed \buchi automata.


==> overview.tex <==
\todo{V: example looks nice. Shall we call the section - Motivating Example?}To motivate our study of repair, we consider the example of a $3$D printer used in manufacturing. The authors of~\cite{confidentiality_printer_side_channel} showed that it was possible to determine intellectual property information by observing the audio output of the system which acts as an acoustic side channel. In our case, we consider a $3$D printer which can print either squares or triangles. The movement of the stepper motors of the printer vary based on the design and this difference in movement leads to the printer producing different sounds. Thus, an intruder may be able to discern the shape being printed by observing the audio output of the system as it acts as an acoustic side-channel. We can model such a system using a \emph{Kripke structure} represented in Figure~\ref{fig:eg_Kripke}. The system initially starts in the state labeled $idle$ and then proceeds to either the state labeled by $\square$ or $\triangle$ depending on whether it is printing a square or triangle after which the motors generate the corresponding sound respectively. It may alternate between these states and thus the evolution of the system can be thought of as an infinite sequence of states that start with the $idle$ state followed by some infinite sequence of $\square$ and $\triangle$.
\begin{figure}[t]
	\begin{subfigure}{0.32\textwidth}
		\centering
		\begin{tikzpicture}[->,thick]
		\node[initial left,cir,initial text={}, label = $idle$]  (s0) {} ;

		\node[cir, label = {$\square$}] at (1,1) (s1) {};
		\node[cir, label = {[yshift = -1.1cm] $\triangle$}] at (1,-1) (s2) {}; 
		\path (s0) edge node{} (s1);
		\path (s0) edge node{} (s2);
		\path (s1) edge[bend right = 20] node{} (s2);
		\path (s2) edge[bend right = 20] node{} (s1);
		\end{tikzpicture}
		\caption{}
		\label{fig:eg_Kripke}
	\end{subfigure}
	\begin{subfigure}{0.32\textwidth}
		\centering
		\begin{tikzpicture}[->,thick]
		\node[initial above, cir, initial text = {}] (p0) {$p_0$}; 
		\node[ cir ] at (1,0) (p1) {$p_1$};
		\node [cir ] at (2,1) (p2) {$p_2$};
		\node [cir] at (2,-1) (p3) {$p_3$};
		\node[cir,accepting] at (3,0) (p4) {$p_4$};
		\path (p0) edge node[midway, above]{$idle$} (p1); 
		\path (p1) edge node[midway, above]{$\triangle$} (p2);
		\path (p2) edge[loop above] node[midway, above] {$\triangle$} (p2);
		\path (p1) edge node[midway, below] {$\square$} (p3); 
		\path (p3) edge[loop below] node[midway, below] {$\square$} (p3);
		\path (p2) edge node[midway, above] {$\square$} (p4);
		\path (p3) edge node[midway, below] {$\triangle$} (p4);
		\path (p4) edge node[midway, above] {$\top$} (p1);
		\end{tikzpicture}
		\caption{}
		\label{fig:omega_prop}
	\end{subfigure}
	\begin{subfigure}{0.32\textwidth}
		\centering
		\begin{tikzpicture}[->,thick]
			\node[initial above,cir,initial text={},accepting] (A) {};
			\path (A) edge[loop right] node [text width=1cm,align=center, right]{$idle|idle, 0$ \\ $\square|\square,0$ \\ $\triangle|\triangle,0$ \\ $\square|\square\triangle,3$ \\ $\square|\square\triangle,3$} (A);
		\end{tikzpicture}
	\caption{}
	\label{fig:eg_transducer}
	\end{subfigure}
%	\vspace{-0.5cm}
	\caption{Krikpe Structure representing the $3$D printer System~(\ref{fig:eg_Kripke}), Transition diagram $B$~(\ref{fig:omega_prop}) specifying the property we would like to satisfy, and Repair machine $T$~(\ref{fig:eg_transducer}).}
	\vspace{-0.5cm}
\end{figure} 


\begin{comment}
	\begin{figure}[t]
	\begin{center}
		\begin{tikzpicture}[->,thick]
		\node[initial above,cir,initial text={},accepting] (A) {};
		\path (A) edge[loop right] node [text width=1cm,align=center, right]{$idle|idle, 0$ \\ $\square|\square,0$ \\ $\triangle|\triangle,0$ \\ $\square|\square\triangle,3$ \\ $\square|\square\triangle,3$} (A);
		\end{tikzpicture}
	\end{center}
	\vspace{-0.5cm}
	\caption{Repair machine $T$}
	\label{fig:eg_transducer}
	\vspace{-0.5cm}
\end{figure}

\end{comment}
Suppose one wishes to hide the fact that the printer's job is to print only one shape, or that it prints only a fixed number of objects of one shape, from an intruder. Such a specification may be modeled by the transition diagram in Figure~\ref{fig:omega_prop}, and one can check if the system satisfies such a specification. In our case, however, we find that our system cannot [cf. Section~\ref{sec:definition}]. As such, we would like to find a way to \emph{repair} our system to ensure that it does indeed satisfy our specification. To do so one may add spurious motor rotations to mimic the other shape, but deciding how to add these is not always trivial as doing so may add a non-trivial cost, and in our case increase the amount of power consumed. We model such changes with the help of the repair machine given in Figure~\ref{fig:eg_transducer}. Intuitively, the edge labels represent what the repair machine reads, its output and the associated overhead cost. For example, the label $\square | \square\triangle,3 $ represents the fact the the repair machine can change the motor rotations corresponding to the square shape with motor rotations that first indicate a square shape followed by rotations that correspond to a triangle shape and doing so incurs a cost of $3$ units of power. Similar to how we associate individual repairs to a cost, we can also associate an infinite sequence of repairs to a cost by aggregating them via a function like the mean or average. For example consider an infinite sequence of repairs whose costs are  represented by the sequence $0,3,0,3,0,3 \ldots $, such an infinite sequence has a total mean cost of $1.5$. Thus, we would like to determine if there exists a strategy to hide the fact of whether a printer prints only one shape while ensuring that the average cost overall is less than $2$ extra units of power. We note that if one were to employ the strategy of adding an extra motor rotation for every shape printed, then the average cost would be $3$ and we cannot accomplish the objective. However, by adding spurious motor rotations at every third shape we can guarantee that the resultant sequence does in fact satisfy the specification with an average cost that is less than $2$.

Similarly, we also study other important aggregator functions such as the discounted sum, the limit supremum and supremum to determine whether there exist strategies to satisfy a specification under a fixed cost overhead. In general, to do so, we consider a product of the system, the repair machine and the specification and try to determine whether such a strategy can be formulated on this product graph.  Lastly, we extend the robustness results from~\cite{concur20} from the context of finite words to that of infinite words.
  

==> threshold-policy-verification.tex <==

\newcommand{\hdelta}{\hat{\delta}}
%\subsection{$v_{T,L}$ for $\mathsf{Sum}$, $\mathsf{DSum}$, $\mathsf{Mean}$, $\mathsf{Sup}$,  $\mathsf{LimSup}$ transducers}
\subsection{Threshold Policy Verification}
Given the Kripke structure $K$ representing the system,\textcolor{blue}{the $\omega$-regular language $L$ capturing undesirable behavior, represented as an NBA $A$}, a repair machine $T$, and a cost semantics $\C \in \{\mathsf{DSum_{\lambda}}, \mathsf{Mean}, \mathsf{Sup}, \mathsf{LimSup}\}$, 
we focus on the threshold verification problem: find a partition of $\Qq_{\geq 0}$  into two sets $\mathbb{G}$ and $\mathbb{B}$, such that none of the traces to system can be rewritten to a word that is in the language of $A$ for all $v \in \mathbb{G}$.
Let $\tau^{*}$ denote the infimum value for which a trace $t \in \Tt_K$ can be rewritten to some word $w \in \Gamma^{\omega}$ such that $w \in L$.
Then, the impair threshold verification problem is solved for any $\tau < \tau^{*}$, as $\sem{T}^\C_{\tau}(t) \not\subseteq L$ for every trace $t \in \Tt_K$.
Thus the set $\mathbb{G} = (0, \tau^{*})$ and the set $\mathbb{B} = [\tau^{*}, \infty)$ and problem reduces to finding the optimal threshold $\tau^{*}$. 

In order to find the optimal threshold $\tau^{*}$, we construct the synchronised product $K{\times}T{\times}A$ as a weighted finite graph $(V,E,W,E,V_I,V_F)$ of the Kripke structure $K$, the repair machine $T$, and the NBA $A$ representing the complement of the language $L$, similar to the case of policy synthesis.
%It is well known that $\omega$-regular languages are closed under complementation and so $\overline{L}$ is $\omega$-regular and admits an NBA $A$ recognizing it.
The sets $V$ and $E$ denote the set of vertices and edges while $W:E \to \Nat$ assigns a weight to every edge. We use $V_I \subseteq V$, $V_F \subseteq V$ to denote the initial and accepting set of vertices of the product. 

We construct a game arena $\Gg = (G, V_{max}, V_{min} )$, with $V_{min} = \emptyset$, $V_{max} = V$ and consider the \buchi game on $\Gg$.
We prune $G$ to contain only those states that are in the winning region of player Min with respect to the \buchi objective, that is, the set of states where player Min has a strategy to enforce visiting \buchi states irrespective of the strategy chosen by the player Max.
As Player Min does not control any vertices, this corresponds to removing all states from which player Max can avoid visiting the accepting states infinitely often.
% \textcolor{blue}{
% \begin{remark}
% We should add that we assume we are given the \buchi automaton $A$ representing the complement of the $\omega$-regular specification.
% This is quite a natural assumption, if, for example the specification is first specified in linear temporal logic.
% In such a case one can first complement the specification in the logic and then directly construct an \buchi automaton representing the complement.
% Our results hold even when this is not given as \buchi automata are closed under complementation, though the complexity results of the following theorems blow-up to $2$-EXPTIME as we need to find the \buchi automaton representing the complement of the given \buchi automaton. 
% \end{remark}
% }
%Intuitively, $K{\times}T{\times}A$ accepts those traces of the system, which have some rewriting that is not in $L$.

%In all of these cases we first prune $G$ to contain only those states which can reach an accepting cycle from the set $V_I$ of initial vertices. 
%\item 	\textbf{Sum Aggregator function}.  
%By definition, the sum aggregator function sums up the costs along an accepting run. If all cycles in $G_{T,A}$ containing 
%a final state from $V_F$  are such that, at least one edge along such cycles have a non zero cost, then $v_{T,L} = \infty$. 
%Therefore we check if there exists some cycle $cyc$ in $G_{T,A}$ containing some final state from $V_F$ such that, all edges 
%on the cycle have cost 0.  If so, we consider all paths $\pi$ from an initial vertex of $G_{T,A}$, ending in a final state 
%appearing in $cyc$.   $v_{T,L}$ is obtained in this case by computing the minimum cost of the path reaching $cyc$ in a final state. 
%%
%%
%%In the case of the sum aggregator function, we note that if we can find a cycle in $G$ with some state in $V_F$ such that the cost of all transitions in the cycle are $0$, then the candidate value of $v_{T,L}$ is the cost of the minimum cost path from some state in $V_I$ to this cycle.
%%Our aim is to find the minimum cost of all such paths which ends in accepting state and that state is a part of cycle having $0$ cost in total. 
%Formally, 
%\[
%v_{T, L} = \min \{c \mid \exists q_0 \in V_I , q_f \in V_F, q_f \text{ is part of a cycle with cost } 0, \text{ and minimum cost of reaching } q_f \text{ from } q_i \text{ is } c\}.
%\]
%If no such cycle exists, then we have $v_{T,L} = \infty$ as any path must visit an accepting cycle infinitely often.

\subsubsection{Computing the Optimal Threshold for $\dsum$-RM.}

%\subparagraph*{Dsum$_\lambda$ Aggregator function}
In the case of a $\dsum$-RM, we claim that the optimal threshold $\tau^{*}$ is the minimum infinite discounted cost path in $K{\times}T{\times}A$.
We show that it may not be possible to achieve this cost, however, for any $\epsilon > 0$, we show the existence of a finite memory strategy that may be used by player Max to guarantee the output word $w$ is in $L$.
Let the value of the minimum discounted cost path be $\tau_{r}$.
To find the value of $\tau_{r}$,  we associate a variable $\Vv_s$, to each vertex $v \in V$, characterizing minimum discounted 
cost among all paths starting from the state $s$. 
The minimum discounted values can then be characterized by the following optimality equation~\cite{PutermanMDP}:
\[
	\Vv_v = \min_{(v, v') \in E} \set{W(v, v') + \lambda \cdot \Vv_{v'}}
\]
A solution of this equation can be computed by solving the following LP:
\begin{align*}
	 \text{ max } \sum_{v \in V} \Vv_v &\text{ subject to: }&
	 \Vv_v \leq W(v,v') + \lambda \Vv_{v} \text{ for all $(v, v') \in E$}.
\end{align*}
To find the minimum discounted infinite cost path, we start from the vertex $v_i \in V_I$ with the least value $\Vv_{v_i}$ compared to all the other vertices in $V_I$. 
Then from all the adjacent vertices $v$, we select the edge with the minimum value of $W'(v_i,v) + \lambda \Vv_{v}$, \textit{i.e.}, $\argmin_{(v_i, v)} \set{ W(v_i,v) + \lambda \Vv_{v}}$. 
This process is continued to get an infinite path which corresponds to the path with the least discounted sum of costs. 
Observe that this path may not satisfy the \buchi condition. 
\begin{figure}[t]
	\begin{center}
	\begin{tikzpicture}[->,thick]
	\node[initial left,cir,initial text={}]  (p0) {$p_0$} ;
	
	\node[cir] at (1,0) (p1) {$p_1$};
	\node[cir, accepting] at (2,0) (p2) {$p_2$};
	\path (p0) edge node[midway, above]{$1$} (p1);
	\path (p1) edge node[midway, above]{$1$} (p2);
	\path (p1) edge[loop above] node[midway,above]{$0$} (p1);
	\path (p2) edge[loop above] node[midway,above]{$1$} (p2);
	\end{tikzpicture}
		\caption{no strategy for optimal $\dsum$ cost.	\label{fig:dsum-inf}}
	\end{center}
\vspace{-0.5cm}
\end{figure}

Consider the graph $K{\times}T{\times}A$ shown in the Figure~\ref{fig:dsum-inf}. 
Suppose there exists a strategy which gives us an accepting path with minimum $\dsum$ cost, and this strategy executes the self loop over $p_1$ $i$ times. 
Since $p_2$ is a \buchi acceptance vertex, it appears infinitely often in this path.
This path will have cost $1+\frac{\lambda^{i+1}}{1-\lambda}$. 
Observe that if we change the strategy and loop over $p_1$ one more time, we get an accepting path with cost
 $1+ \frac{\lambda^{i+2}}{1-\lambda}$, strictly smaller than the earlier one,  contradicting  the assumption that there exists an optimal strategy.

\begin{theorem}
\label{thm:dsum-verif}
The optimal threshold $\tau^{*}$ for $\dsum$-RMs can be computed in P. 
\end{theorem}
\begin{proof}
First we show that the optimal threshold $\tau^{*}$ is the minimum infinite discounted cost path.
Let value of the minimum discounted cost path be $\tau_{r}$, and let us suppose $\tau^{*} < \tau_{r}$, then there must exist a trace $t \in \Tt_K$ and a word $w \in L$, such that $\sem{T}^{\mathsf{DSum}}_{*}(t,w) < \tau_{r}$. 
As the trace $t$ has a rewriting that is in $L$, it must be accepted by $K{\times}T{\times}A$, however if $t$ is accepted by $K{\times}T{\times}A$, then it must follow an infinite path in $K{\times}T{\times}A$.
The discounted cost of this infinite path must be at least as large as $\tau_{r}$ which is a contradiction.

 Let $W$ be an upper bound on the weights in the graph $K{\times}T{\times}A$. Then for any $\epsilon > 0$, there exists some $k\in \mathbb{N}$ such that $\lambda^{k} \frac{W}{1 - \lambda} \leq \epsilon$.  
 We follow the discounted policy obtained from the above optimality equation for $k$ steps and then choose an arbitrary policy to an accepting cycle and follow an accepting cycle thereafter. 
 It follows that the resulting path is an accepting path with cost bounded by $\tau^{*} + \epsilon$.
  It is easy to see this : consider a path with all the edges having cost $W$. 
 The discounted sum for this path is $\frac{W}{1-\lambda}$. 
 If we follow the discounted strategy for the first $k$ steps on the path as defined above, then any of its infinite extensions will cost no more than $\tau^{*} + \lambda^k \frac{W}{1-\lambda} \leq \tau^{*} + \epsilon$. 
 We note that this is an accepting path in $K{\times}T{\times}A$, and so for any $\epsilon > 0$, $\tau_{r} + \epsilon \in \mathbb{B}$ .
 
 We note that the size of the graph $K{\times}T{\times}A$ is polynomial in $K,T$ and $A$.
 Solving the \buchi game on this graph and the above linear program is in $P$.
%  Hence, finding $\tau^{*}$ is in P.
% However, computing the automaton $A$ requires EXPTIME~\cite{safra_1988_complexity} and hence the overall complexity is in EXPTIME.
 \qed
\end{proof}
\vspace{0.5em}

% Let $W$ be an upper bound on the weights in the graph $G$, then 
% for any $\epsilon > 0$, there exists some $k\in \mathbb{N}$ such that $\lambda^{k} \frac{W}{1 - \lambda} \leq \epsilon$. 
%Thus, to approximate $v_{T,L} + \epsilon$, we follow the above strategy for $k$ steps and then take the shortest path to an accepting cycle and follow the cycle thereafter. 
%We follow the optimal discounted strategy for $k$ steps and then choose an arbitrary strategy 
%to an accepting cycle and follow an accepting cycle thereafter. 
%It follows that the resulting path is an accepting path with cost bounded by $v_{T, L} + \epsilon$.
%It is easy to see: assume in worst case, there exists a path with all the edges having cost $W$. 
%The discounted sum for this path is $\frac{W}{1-\lambda}$. 
%Thus if we follow optimal strategy for k steps, then any of its infinite extensions will cost no more than $v_{T, L} + \lambda^k \frac{W}{1-\lambda} \leq v_{T, L} + \epsilon$. 
% Thus, after taking $k$ steps from this strategy, even if all the edges 
% seen after have a weight of $W$ the total cost is at most $v_{T, L} + \epsilon$.   



\subsubsection{Optimal Threshold for $\mean$-RM.}

In the case of the $\mathsf{Mean}$ aggregator function, we note that only those edges that are visited infinitely often have an effect on the cost.
We say that a cycle is accepting if there exists some vertex $v \in V_F$ that occurs in the cycle.  
We let $C_1$ denote the least average cost cycle that can be reached and is reachable from some accepting cycle $C_2$. 
We use $d_1$ and $d_2$ to denote the total cost of these cycles and $n_1$ and $n_2$ to be the number of edges in each of them respectively.
We then show that $\tau^{*}$ is the mean value of cycle $C_1$.
\begin{theorem}
\label{thm:mean-verif}
The  threshold $\tau^{*}$ for $\mean$-RMs can be computed in P.
\end{theorem}
\begin{proof}
    First we claim that the optimal threshold $\tau^{*}$ is the value of the average cost of cycle $C_1$, where $C_1$ is the least cost cycle that can be reached and is reachable from some accepting cycle $C_2$.
	Suppose $\tau^{*}$ is lesser than the mean cost of $C_1$. 
	Then there must exist some edges that are visited infinitely often such that their average cost is less than the average cost of $C_1$.
	The graph $K{\times}T{\times}A$ has a finite number of edges, so these edges must be a part of some cycle as they are visited infinitely often. 
	However this cycle must also be reachable and reach some accepting cycle.
	This must imply that there exists a cycle with an average cost that is strictly less than the average cost of $C_1$ which contradicts our assumption.
    If $C_1$ and $C_2$ are the same, \textit{i.e.}, $C_1$ is an accepting cycle then the value of $\tau^{*}$ is equal to the average cost of $C_1$. Without loss of generality we can assume that the two cycles $C_1$ and $C_2$ are incident at a common point (by collapsing the path in between them). 
    We can collapse cycles $C_1$ and $C_2$ into a common point by extending the cycle $C_2$ to constitute a larger cycle that passes through $C_1$ and returns to $C_2$. 
	Moreover, it does not affect the least mean cost of the graph.
	An example for the same is shown in Appendix~\ref{app:fig:cycle}.
	We now prove $\tau^{*} = \frac{d_1}{n_1}$ by giving a strategy to find an accepting path of the graph with mean cost as $\frac{d_1}{n_1}$.
	To find the value of $\tau^{*}$ when $C_1$ and $C_2$ are not the same, we consider the strategy of cycling between $C_1$ and $C_2$ in rounds. At any round $i$, we cycle $2^{i}$ many times in $C_1$ and once in cycle $C_2$. We can write the value of the average computed after round $i$ as 
	
\[a_i = \dfrac{(1 + 2 + \ldots + 2^{i}) d_1 + i \cdot d_2 }{(1 + 2 + \ldots + 2^{i}) n_1 + i\cdot n_2} = \dfrac{(2^{i+1} - 1) d_1 + i\cdot d_2 }{(2^{i+1} - 1) n_1 + i\cdot n_2} \]

From the properties of limits of real sequences we note that the sequence $a_0, a_1, \ldots $ converges to $\frac{d_1}{n_1}$, and thus we have $\tau^{*} = \frac{d_1}{n_1}$.
We note that the sequence $a_1, a_2 \ldots$ is a Cauchy sequence and so for any $\epsilon > 0$, there exists some $M$ such that for all $i,j \geq M$, we have $|a_i - a_j| \leq \epsilon$. 
Thus for any $\epsilon > 0$, there exists some $k$ such that $a_k = \tau^{*}+ \epsilon$. 
We can thus follow a policy where we alternate cycling $2^{k+1}$ times in $C_1$ and once in $C_2$ to approximate $\tau^{*}$ to within $\epsilon$.

Secondly, the graph $K{\times}T{\times}A$ is polynomial in the sizes of $K,T$ and $A$.
We find the least mean cost cycle that is co-accessible from an accepting vertex as follows.
First, we prune the graph $K{\times}T{\times}A$ to contain only those vertices that are co-accessible from an accepting vertex, this is polynomial as it relies on solving reachability from and to all vertices.
Secondly we use Karp's algorithm~\cite{karp_mean_value} to find the cost of the least mean cycle and note that this cycle can be reached and is reachable from an accepting vertex. 
The mean value of this cycle corresponds to the optimal threshold and so this can be done in P.
%  Hence, finding $\tau^{*}$ is in P.
% However, we take EXPTIME to compute the NBA $A$ representing the complement of the language $L$ and so the overall complexity is in EXPTIME.
\qed
\end{proof}

%To note that the above series converges we show that the limit as $i$ approaches $\infty$ is defined.
%We have,
%\[\lim_{i \to \infty} a_i = \lim_{i \to \infty } \dfrac{(2^{i+1} - 1) c_1 + ic_2 }{(2^{i+1} - 1) n_1 + in_2} = \lim_{i \to \infty} \dfrac{c_1 + \frac{i}{2^{i+1}} \cdot c_2 - \frac{c_1}{2^{i+1}} }{ n_1 + \frac{i}{2^{i+1}} \cdot n_2 - \frac{n_1}{2^{i+1}} } \]


\subsubsection{Optimal Thresholds for $\supf$-RMs and $\limsupf$-RMs.}
%\subparagraph*{Sup and LimSup aggregator functions}
For the $\mathsf{Sup}$ aggregator function, let $S$ be the set of values $c_i$ such that $c_i$ is the supremum of the cost of some lasso that starts from some $v_i \in V_I$ and cycles in a loop containing some $v_f \in V_F$. Let $k$ be the least element in $S$. We claim $\tau^{*} = k$.
\begin{theorem}
\label{thm:sup-verif}
The threshold  $\tau^{*}$ for $\supf$ and $\limsupf$-RMs can be computed in P.
\end{theorem}
The proof of Theorem~\ref{thm:sup-verif} is found in Appendix~\ref{ap:sup-verif}.

\textcolor{blue}{
Finally, we summarize our results for impair verification in Table~\ref{tab:verif_summary}.
}
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline & &\\
     cost semantics & exact or $\epsilon$-optimal & Complexity \\
     \hline & & \\
     $\dsum$ & $\epsilon$-optimal & P \\
     $\mean$ (infinite memory) & exact & P \\
     $\mean$ (finite memory) & $\epsilon$-optimal & P \\
    $\supf$ & exact & P \\
    $\limsupf$ & exact & P \\
    \hline
    \end{tabular}
    \caption{Summary of finding the thresholds for different cost semantics from Section~\ref{sec:verification}}
    \label{tab:verif_summary}
\end{table}


==> threshold-policy.tex <==

%\section{Robustness Verification}
%
%We define the following problems concerning the robustness verification of $C$-transducers:
%Given a threshold $v \in \Qq$, a $C$-transducer $T$ and an $\omega$-regular language 
%$L \subseteq \Sigma^\omega$, a word $u \in \dom(T)$ is said to be $v$-robust 
%if $T_{\leq v}(u) \subseteq L$.
%In other words, all its outputs are at most $v$ far.
%A language $N \subseteq \Sigma^\omega$ is said to be $v$-robust if $N \cap \dom(T)$ 
%contains only $v$-robust words.
%$v$-robust kernel of $T$ denoted as $\rob_T(v, L)$, is defined as set of 
%$v$-robust words i.e. $\{u \in \dom(T) \mid T_{\leq v}(u) \subseteq L\}$.
%We study the \emph{robust kernel synthesis problem} in the following sections.
%
%Given a $C$-transducer $T$, $\omega$-regular languages $N, L \subseteq \Sigma^\omega$ as 
%NBA, the \emph{threshold synthesis problem} is to output a partition of the set 
%of thresholds $\Qq_{\geq 0}$ as good ($G$) and bad ($B$) thresholds.
%$$G = \{v \in \Qq_{\geq 0} \mid N \subseteq \rob_T(v, L)\} \text{~and~} 
%B = \{v \in \Qq_{\geq 0} \mid N \nsubseteq \rob_T(v, L)\}$$

%This reverses in the case of repair verification, where restricting the value of $v$ to a lower value reduces the number of possible strategies.  
%Here we let $v_{K, L, T}$ denote the least value $v$, for which some trace $t \in \Tt(k)$ can be rewritten to some word $w \in \Gamma^{\omega}$, such that $w \notin L$.
%Therefore the sets $\mathbb{G} = (0, v_{K, L, T})$ and $\mathbb{B} = [v_{K, L, T}, \infty)$.
%Thus the problems of threshold policy synthesis and verification reduce to finding the value $v_{K, L, T}$. 

%To help determine this, we make use of the \emph{synchronized product} $G$  of the Kripke Structure $K$ representing the system, the repair machine $T$, and either the \buchi automaton $A$ representing the complement of $L$ or the \buchi automaton $B$ representing $L$. 
%It is well known that $\omega$-regular languages are closed under complementation and so there exists a \buchi automaton representing the complement of the language $L$. 
%Formally, the synchronized product $G = (V,E,W': E \to \Nat)$ is a weighted graph with $V$ denoting the set of vertices, $E$ the set of edges and the weight function $W'$ that assigns to each edge a weight %from $\Nat$. We use  $V_I \subseteq V$ and $V_F \subseteq V$ to denote the initial and accepting set of vertices of this synchronized product. 
%The details of this construction are presented in the Appendix.
%In either case, we then consider the \buchi game on $G$ and prune it to contain only those states that are in the winning region of player Min with respect to the \buchi objective, that is, the set of states where player Min has a strategy to enforce visiting \buchi states irrespective of the strategy chosen by the player Max.

%\smallskip

%\noindent\textbf{Synchronizing $T$ and $A$}. 
% I think we can change this to a product of the complement and the transducer 

%\noindent \textbf{Computing $v_{T,L}$ from $G_{T,A}$}. 
%We want to find $v_{T,L}$ using $G_{T,A}$.  
%Recall that $v_{T,L}$ is defined as $\inf\{v \in \Qq_{\geq 0} \mid \dom(T) \nsubseteq \rob_T(v, L)\}$. Using $G_{T,A}$ we show the following. %(Proof in Appendix~\ref{app:lem:vtl}).
%\begin{lemma}\label{lem:vtl} The value $v_{K, L, T}$ is equal to the infimum of all values $C(\pi)$ such that the path $\pi$ begins at some initial vertex $s_0 \in V_I$ and cycles on some state $s_F \in V_F$ infinitely often. 
%%$v_{T,L} = \inf\{C(\pi) \mid$  there is an initial vertex  $s_0 \in V_I$,  a final vertex $s_f \in V_F$ and a path  $\pi$ from $s_0$ which visits  $s_f$ infinitely often$\} $.	
%\end{lemma}

